Enhancing Clinical Support for Breast Cancer with Deep Learning Models using Synthetic Correlated Diffusion Imaging

Breast cancer is the second most common type of cancer in women in Canada and the United States, representing over 25\% of all new female cancer cases. As such, there has been immense research and progress on improving screening and clinical support for breast cancer. In this paper, we investigate enhancing clinical support for breast cancer with deep learning models using a newly introduced magnetic resonance imaging (MRI) modality called synthetic correlated diffusion imaging (CDI$^s$). More specifically, we leverage a volumetric convolutional neural network to learn volumetric deep radiomic features from a pre-treatment cohort and construct a predictor based on the learnt features for grade and post-treatment response prediction. As the first study to learn CDI$^s$-centric radiomic sequences within a deep learning perspective for clinical decision support, we evaluated the proposed approach using the ACRIN-6698 study against those learnt using gold-standard imaging modalities. We find that the proposed approach can achieve better performance for both grade and post-treatment response prediction and thus may be a useful tool to aid oncologists in improving recommendation of treatment of patients. Subsequently, the approach to leverage volumetric deep radiomic features for breast cancer can be further extended to other applications of CDI$^s$ in the cancer domain to further improve clinical support.

==> backup-bib.tex <==
@String(PAMI = {IEEE Trans. Pattern Anal. Mach. Intell.})
@String(IJCV = {Int. J. Comput. Vis.})
@String(CVPR= {IEEE Conf. Comput. Vis. Pattern Recog.})
@String(ICCV= {Int. Conf. Comput. Vis.})
@String(ECCV= {Eur. Conf. Comput. Vis.})
@String(NIPS= {Adv. Neural Inform. Process. Syst.})
@String(ICPR = {Int. Conf. Pattern Recog.})
@String(BMVC= {Brit. Mach. Vis. Conf.})
@String(TOG= {ACM Trans. Graph.})
@String(TIP  = {IEEE Trans. Image Process.})
@String(TVCG  = {IEEE Trans. Vis. Comput. Graph.})
@String(TMM  = {IEEE Trans. Multimedia})
@String(ACMMM= {ACM Int. Conf. Multimedia})
@String(ICME = {Int. Conf. Multimedia and Expo})
@String(ICASSP=	{ICASSP})
@String(ICIP = {IEEE Int. Conf. Image Process.})
@String(ACCV  = {ACCV})
@String(ICLR = {Int. Conf. Learn. Represent.})
@String(IJCAI = {IJCAI})
@String(PR   = {Pattern Recognition})
@String(AAAI = {AAAI})
@String(CVPRW= {IEEE Conf. Comput. Vis. Pattern Recog. Worksh.})
@String(CSVT = {IEEE Trans. Circuit Syst. Video Technol.})

@String(SPL	= {IEEE Sign. Process. Letters})
@String(VR   = {Vis. Res.})
@String(JOV	 = {J. Vis.})
@String(TVC  = {The Vis. Comput.})
@String(JCST  = {J. Comput. Sci. Tech.})
@String(CGF  = {Comput. Graph. Forum})
@String(CVM = {Computational Visual Media})


@String(PAMI  = {IEEE TPAMI})
@String(IJCV  = {IJCV})
@String(CVPR  = {CVPR})
@String(ICCV  = {ICCV})
@String(ECCV  = {ECCV})
@String(NIPS  = {NeurIPS})
@String(ICPR  = {ICPR})
@String(BMVC  =	{BMVC})
@String(TOG   = {ACM TOG})
@String(TIP   = {IEEE TIP})
@String(TVCG  = {IEEE TVCG})
@String(TCSVT = {IEEE TCSVT})
@String(TMM   =	{IEEE TMM})
@String(ACMMM = {ACM MM})
@String(ICME  =	{ICME})
@String(ICASSP=	{ICASSP})
@String(ICIP  = {ICIP})
@String(ACCV  = {ACCV})
@String(ICLR  = {ICLR})
@String(IJCAI = {IJCAI})
@String(PR = {PR})
@String(AAAI = {AAAI})
@String(CVPRW= {CVPRW})
@String(CSVT = {IEEE TCSVT})


@inproceedings{3d-cnn-bc-detect,
  author   = "Amin Ul Haq and Jian Ping Li and Abdus Saboor and Jalaluddin Khan and Wang Zhou and Tao Jiang and Mordecai F. Raji and Samad Wali",
  title    = "3DCNN: Three-Layers Deep Convolutional Neural Network Architecture for Breast Cancer Detection using Clinical Image Data",
  journal  = "17th International Computer Conference on Wavelet Active Media Technology and Information Processing (ICCWAMTIP)",
  booktitle = "17th International Computer Conference on Wavelet Active Media Technology and Information Processing (ICCWAMTIP)",
  series    = "ICCWAMTIP",
  year      = 2020,
  publisher = "IEEE",
  address   = "Chengdu, China"
}

@article{3d-resnet-seminal-paper,
  author   = "Kensho Hara and Hirokatsu Kataoka and Yutaka Satoh",
  title    = "Learning Spatio-Temporal Features with 3D Residual Networks
for Action Recognition",
  journal   = {CoRR},
  volume    = {abs/1708.07632},
  year      = {2017},
  url       = {http://arxiv.org/abs/1708.07632},
  eprinttype = {arXiv},
  eprint    = {1708.07632},
  timestamp = {Mon, 13 Aug 2018 16:47:12 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1708-07632.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{8915701,  
    author={Fan, Ming and Yuan, Wei and Zhao, Wenrui and Xu, Maosheng and Wang, Shiwei and Gao, Xin and Li, Lihua},  
    journal={IEEE Journal of Biomedical and Health Informatics},   
    title={Joint Prediction of Breast Cancer Histological Grade and Ki-67 Expression Level Based on DCE-MRI and DWI Radiomics},  
    year={2020},  
    volume={24},  
    number={6},  
    pages={1632-1642},  
    doi={10.1109/JBHI.2019.2956351}
}

@article{acrin6657-predict,
  author   = "Nola M. Hylton and Jeffrey D. Blume and Wanda K. Bernreuter and Etta D. Pisano and Mark A. Rosen and Elizabeth A. Morris and Paul T. Weatherall and Constance D. Lehman and Gillian M. Newstead and Sandra Polin and Helga S. Marques and Laura J. Esserman and Mitchell D. Schnall",
  title    = "Locally Advanced Breast Cancer: MR Imaging for Prediction of Response to Neoadjuvant Chemotherapy—Results from ACRIN 6657/I-SPY TRIAL",
  journal  = "Radiology",
  year     = 2012,
  volume   = "263",
  number = "3",
  pages    = "663--672",
}

@article{acrin6698-data-1,
  author   = "S. C. Partridge and Z. Zhang and D. C. Newitt and J. E. Gibbs and T. L. Chenevert and M. A. Rosen and P. J. Bolan and H. S. Marques and J. Romanoff and L. Cimino and B. N. Joe and H. R. Umphrey and H. Ojeda-Fournier and B. Dogan and K. Oh and H. Abe and J. S. Drukteinis and L. J. Esserman and N. M. Hylton",
  title    = "Diffusion-weighted MRI Findings Predict Pathologic Response in Neoadjuvant Treatment of Breast Cancer: The ACRIN 6698 Multicenter Trial",
  journal  = "Radiology",
  year     = 2018,
  volume   = "289",
  number = "3",
  pages    = "618--627",
}

@article{acrin6698-data-2,
  author   = "D. C. Newitt and Z. Zhang and J. E. Gibbs and S. C. Partridge and T. L. Chenevert and M. A. Rosen and P. J. Bolan and H. S. Marques and S. Aliu and W. Li and L. Cimino and B. N. Joe and H. Umphrey and H. Ojeda‐Fournier and B. Dogan and K. Oh, H. Abe and J. Drukteinis and L. J. Esserman",
  title    = "Test–retest repeatability and reproducibility of ADC measures by breast DWI: Results from the ACRIN 6698 trial",
  journal  = "Journal of Magnetic Resonance Imaging",
  year     = 2018,
  volume   = "49",
  number = "6",
  pages    = "1617-1628",
}

@article{acrin6698-data-3,
  author   = "D. C. Newitt and S. C. Partridge and Z. Zhang, J. Gibbs, T. Chenevert and M. Rosen and P. Bolan and H. Marques and J. Romanoff and L. Cimino and B. N. Joe and H. Umphrey and H. Ojeda-Fournier and B. Dogan and K. Y. Oh and H. Abe and J. Drukteinis and L. J. Esserman and N. M. Hylton",
  title    = "ACRIN 6698/I-SPY2 Breast DWI [Data set]",
  journal  = "The Cancer Imaging Archive",
  year     = 2021
}

@article{acrin6698-data-4,
  author   = "K. Clark and B. Vendt and K. Smith and J. Freymann and J. Kirby and P. Koppel and S. Moore and S. Phillips and D. Maffitt and M. Pringle and L. Tarbox and F. Prior",
  title    = "The Cancer Imaging Archive (TCIA): Maintaining and Operating a Public Information Repository",
  journal  = "Journal of Digital Imaging",
  year     = 2013,
  volume   = "26",
  number = "6",
  pages    = "1045-1057",
}

@misc{ai-transform-breast,
  title = "Using A.I. to Transform Breast Cancer Care",
  author = "{Susan Gubar}",
  howpublished = "\url{https://www.nytimes.com/2019/10/24/well/live/machine-intelligence-AI-breast-cancer-mammogram.html}",
  year = 2019,
  note = "Accessed: 2022-06-02"
}

@misc{american-cancer-death,
  title = "Key Statistics for Breast Cancer",
  author = "{American Cancer Society}",
  howpublished = "\url{https://www.cancer.org/cancer/breast-cancer/about/how-common-is-breast-cancer.html}",
  year = 2023,
  note = "Accessed: 2023-01-12"
}

@misc{bc-grading,
  title = "Grading breast cancer",
  author = "{Canadian Cancer Society}",
  howpublished = "\url{https://cancer.ca/en/cancer-information/cancer-types/breast/grading}",
  note = "Accessed: 2022-12-10"
}

@misc{bc-grading2,
  title = "Breast Cancer Grade",
  author = "{American Cancer Society}",
  howpublished = "\url{https://www.cancer.org/cancer/breast-cancer/understanding-a-breast-cancer-diagnosis/breast-cancer-grades.html}",
  note = "Accessed: 2022-12-10"
}

@misc{bc-types,
  title = "Types of Breast Cancer",
  author = "{American Cancer Society}",
  howpublished = "\url{https://www.cancer.org/cancer/breast-cancer/about/types-of-breast-cancer.html}",
  year = 2022,
  note = "Accessed: 2022-12-14"
}

@article{biomarkers-predicting,
  author   = "Xiaoxian (Bill) Li and Uma Krishnamurti and Shristi Bhattarai and Sergey Klimov and Michelle D. Reid and Ruth O’Regan and Ritu Aneja",
  title    = "Biomarkers Predicting Pathologic Complete Response to Neoadjuvant Chemotherapy in Breast Cancer",
  journal  = "American Journal of Clinical Pathology",
  year     = 2016,
  volume   = "145",
  number = "6",
  pages    = "871--878",
}

@misc{biospy-pain,
  title = "How Painful is Breast Cancer Biopsy \& How Long Does It Take To Recover",
  author = "{Valley County Health System}",
  howpublished = "\url{https://www.valleycountyhealthsystem.org/about-us/news-events/blog/how-painful-is-breast-cancer-biopsy-and-how-long-does-it-take-to-recover.html}",
  year = 2020,
  note = "Accessed: 2022-12-10"
}

@misc{breast-biopsy-costs,
  title = "Breast Biopsy",
  author = "{MDsave}",
  howpublished = "\url{https://www.mdsave.com/procedures/breast-biopsy/d78af5cf}",
  note = "Accessed: 2022-12-14"
}


@misc{breast-cancer-staging,
  title = "About breast cancer staging and grades",
  author = "{Cancer Research UK}",
  howpublished = "\url{https://www.cancerresearchuk.org/about-cancer/breast-cancer/stages-types-grades/about-breast-cancer-staging-grades}",
  note = "Accessed: 2022-12-10"
}

@inproceedings{cancer-net-bca,
	title = {Cancer-Net BCa: Breast Cancer Pathologic Complete Response Prediction using Volumetric Deep Radiomic Features from Synthetic Correlated Diffusion Imaging},
	author = {Tai, Chi-en Amy and Hodzic, Nedim and Flanagan, Nic and Gunraj, Hayden and Wong, Alexander},
	booktitle = {Conference and Workshop on Neural Information Processing Systems (NeurIPS)},
    	series = {Medical Imaging Meets NeurIPS Workshop (MED-NeurIPS)},
	year = {2022},
	url = {https://arxiv.org/abs/2211.05308}
}

@misc{cancer-stages,
  title = "Breast Cancer - Stages",
  author = "{Cancer.NET}",
  howpublished = "\url{https://www.cancer.net/cancer-types/breast-cancer/stages}",
  year = 2021,
  note = "Accessed : 2022-12-10"
}

@misc{cancer-stats,
  title = "Breast Cancer - Statistics",
  author = "{Cancer.NET}",
  howpublished = "\url{https://www.cancer.net/cancer-types/breast-cancer/statistics}",
  year = 2023,
  note = "Accessed : 2023-06-10"
}

@article{comp-tumors,
    title = {Using computer-extracted image phenotypes from tumors on breast magnetic resonance imaging to predict breast cancer pathologic stage},
    journal={ACS Journals},
    volume = {122},
    number = {5},
    pages={748-757},
    year = {2016},
    url = {https://acsjournals.onlinelibrary.wiley.com/doi/full/10.1002/cncr.29791},
    author = {Elizabeth S. Burnside and Karen Drukker and Hui Li and Ermelinda Bonaccio and Margarita Zuley and Marie Ganott and Jose M. Net and Elizabeth J. Sutton and Kathleen R. Brandt and Gary J. Whitman and Suzanne D. Conzen and Li Lan and Yuan Ji and Yitan Zhu and Carl C. Jaffe and Erich P. Huang and John B. Freymann and Justin S. Kirby and Elizabeth A. Morris and Maryellen L. Giger},
}

@article{cost-effectiveness-nac,
  author   = "Natalia Kunst and Shi-Yi Wang and Annette Hood and Sarah S Mougalian and Michael P DiGiovanna and Kerin Adelson and Lajos Pusztai",
  title    = "Cost-Effectiveness of Neoadjuvant-Adjuvant Treatment Strategies for Women With ERBB2 (HER2)–Positive Breast Cancer",
  journal  = "JAMA Network Open",
  year     = 2020,
  volume   = "3",
  number = "11",
}

@article{dce,
    title = {Joint Prediction of Breast Cancer Histological Grade and Ki-67 Expression Level Based on DCE-MRI and DWI Radiomics},
    journal={IEEE Journal of Biomedical and Health Informatics},
    volume = {24},
    number = {6},
    pages = {1632-1642},
    year = {2020},
    url = {https://ieeexplore.ieee.org/abstract/document/8915701},
    author = {Ming Fan and Wei Yuan and Wenrui Zhao and Maosheng Xu and Shiwei Wang and Xin Gao and Lihua Li},
}

@article{doi:10.1148/rg.296095521,
    author = {Qayyum, Aliya},
    title = {Diffusion-weighted Imaging in the Abdomen and Pelvis: Concepts and Applications},
    journal = {RadioGraphics},
    volume = {29},
    number = {6},
    pages = {1797-1810},
    year = {2009},
    doi = {10.1148/rg.296095521},
    note ={PMID: 19959522},
    URL = {https://doi.org/10.1148/rg.296095521},
    eprint = {https://doi.org/10.1148/rg.296095521}
}

@article{dwi-prediction,
    title = {Can diffusion-weighted imaging predict tumor grade and expression of Ki-67 in breast cancer? A multicenter analysis},
    journal = {Breast Cancer Research},
    volume = {20},
    number = {58},
    year = {2018},
    url = {https://breast-cancer-research.biomedcentral.com/articles/10.1186/s13058-018-0991-1},
    author = {Alexey Surov and Paola Clauser and Yun-Woo Chang and Lihua Li and Laura Martincich and Savannah C. Partridge and Jin You Kim and Hans Jonas Meyer and Andreas Wienke},
}

@article{elastography,
    title = {Strain Elastography for Prediction of Breast Cancer Tumor Grades},
    journal = {Journal of Ultrasound in Medicine},
    volume = {35},
    number = {1},
    year = {2014},
    url = {https://onlinelibrary.wiley.com/doi/abs/10.7863/ultra.33.1.129},
    author = {Joseph R. Grajo and Richard G. Barr},
}

@article{extended-apriori-prediction,
  author   = "Hadi Moghadas-Dastjerdi and Hira R. Sha-E-Tallat and Lakshmanan Sannachi and Laurentius O. Osapoeta and Ali Sadeghi-Naini and Gregory J. Czarnota",
  title    = "A priori prediction of tumour response to neoadjuvant chemotherapy in breast cancer patients using quantitative CT and machine learning",
  journal  = "Scientific Reports",
  year     = 2020,
  volume   = "10",
  pages    = "1188--1199",
}

@article{grading-future,
  author   = "C. van Dooijeweert and P.J. van Diest and I.O. Ellis",
  title    = "Grading of invasive breast carcinoma: the way forward",
  journal  = "Virchows Archiv",
  volume    = {480},
  year      = {2022},
  pages    = {33-43},
  url       = {https://link.springer.com/article/10.1007/s00428-021-03141-2}
}

@misc{https://doi.org/10.48550/arxiv.1606.05718,
  doi = {10.48550/ARXIV.1606.05718},
  url = {https://arxiv.org/abs/1606.05718},
  author = {Wang, Dayong and Khosla, Aditya and Gargeya, Rishab and Irshad, Humayun and Beck, Andrew H.},
  keywords = {Quantitative Methods (q-bio.QM), Computer Vision and Pattern Recognition (cs.CV), FOS: Biological sciences, FOS: Biological sciences, FOS: Computer and information sciences, FOS: Computer and information sciences},
  title = {Deep Learning for Identifying Metastatic Breast Cancer},
  publisher = {arXiv},
  year = {2016},
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@article{human-judgement-problem,
  author   = "Donald A. Redelmeier and Lorraine E. Ferris and Jack V. Tu and Janet E. Hux and Michael J. Schull",
  title    = "Problems for clinical judgement: introducing cognitive psychology as one more basic science",
  journal  = "Canadian Medical Association Journal",
  year     = 2001,
  volume   = "164",
  number = "3",
  pages    = "358--360",
}

@article{image-analysis,
    title = {Image analysis with deep learning to predict breast cancer grade, ER status, histologic subtype, and intrinsic subtypes},
    journal={npj Breast Cancer},
    volume = {4},
    number = {30},
    year = {2018},
    url = {https://www.nature.com/articles/s41523-018-0079-1},
    author = {Heather D. Couture and Lindsay A. Williams and Joseph Geradts and Sarah J. Nyante and Ebonee N. Butler and J. S. Marron and Charles M. Perou and Melissa A. Troester and Marc Niethammer},
}

@article{MARTINEZHERAS2021490,
    title = {Diffusion-Weighted Imaging: Recent Advances and Applications},
    journal = {Seminars in Ultrasound, CT and MRI},
    volume = {42},
    number = {5},
    pages = {490-506},
    year = {2021},
    note = {Advances in Neuroradiology I},
    issn = {0887-2171},
    doi = {https://doi.org/10.1053/j.sult.2021.07.006},
    url = {https://www.sciencedirect.com/science/article/pii/S0887217121000846},
    author = {Eloy Martinez-Heras and Francesco Grussu and Ferran Prados and Elisabeth Solana and Sara Llufriu}
}

@inproceedings{ml-qCT,
  author   = "Hadi Moghadas-Dastjerdi and Hira R. Sha-E-Tallat and Lakshmanan Sannachi and Laurentius O. Osapoeta and Ali Sadeghi-Naini and Gregory J. Czarnota",
  title    = "Machine Learning-Based A Priori Chemotherapy Response Prediction in Breast Cancer Patients using Textural CT Biomarkers",
  journal  = "42nd Annual International Conference of the IEEE Engineering in Medicine \& Biology Society (EMBC)",
  booktitle = "42nd Annual International Conference of the IEEE Engineering in Medicine \& Biology Society (EMBC)",
  series    = "EMBC",
  year      = 2020,
  publisher = "IEEE",
  address   = "Montreal, QC, Canada"
}

@article{nac-bc-r,
  author   = "A. Fangberget and L. B. Nilsen and K. H. Hole and M. M. Holmen and O. Engebraaten and B. Naume and H.-J. Smith and D. R. Olsen and T. Seierstad",
  title    = "Neoadjuvant chemotherapy in breast cancer-response evaluation and prediction of response to treatment using dynamic contrast-enhanced and diffusion-weighted MR imaging",
  journal  = "European Radiology",
  year     = 2011,
  volume   = "21",
  pages    = "1188--1199",
}

@article{nac-human-recommendation,
  author   = "Shahla Masood",
  title    = "Neoadjuvant chemotherapy in breast cancers",
  journal  = "Womens Health",
  year     = 2016,
  volume   = "12",
  number = "5",
  pages    = "480--491",
}

@misc{nac-side-effects,
  title = "Neoadjuvant chemotherapy: Benefits, side effects, and drugs",
  author = "{Lindsey Todd}",
  howpublished = "\url{https://www.medicalnewstoday.com/articles/neoadjuvant-chemotherapy}",
  year = 2021,
  note = "Accessed: 2022-06-02"
}

@misc{pcr-bc,
  title = "Pathologic Complete Response to Targeted Therapy Before Surgery Linked to Better Survival for Early-Stage HER2-Positive Breast Cancer",
  author = "{Jamie DePolo}",
  howpublished = "\url{https://www.breastcancer.org/research-news/neoadjuvant-pcr-linked-to-better-survival}",
  year = 2020,
  note = "Accessed: 2022-06-02"
}

@article{predicting-post-neoadjuvant,
  author   = "Richard Ha and Peter Chang and Jenika Karcich and Simukayi Mutasa and Eduardo Pascual Van Sant and Eileen Connolly and Christine Chin and Bret Tabacka and Michael Z. Liu and Sachin Jambawalikar",
  title    = "Predicting Post Neoadjuvant Axillary Response Using a Novel Convolutional Neural Network Algorithm",
  journal  = "Annals of Surgical Oncology",
  year     = 2018,
  volume   = "25",
  pages    = "3037--3043",
}

@article{prediction-dwi-mrs,
  author   = "Hee Jung Shin and Hyeon-Man Baek and Jin-Hee Ahn and Seunghee Baek and Hyunji Kim and Joo Hee Cha and Hak Hee Kim",
  title    = "Prediction of pathologic response to neoadjuvant chemotherapy in patients with breast cancer using diffusion-weighted imaging and MRS",
  journal  = "NMR Biomedical",
  year     = 2012,
  volume   = "25",
  number = "12",
  pages    = "1349--1359",
}

@inproceedings{prediction-pcr-3dcnn,
  author   = "Hongyi Duanmu and Pauline Boning Huang and Srinidhi Brahmavar and Stephanie Lin and Thomas Ren and Jun Kong and Fusheng Wang and Tim Q. Duong",
  editor="Martel, Anne L. and Abolmaesumi, Purang and Stoyanov, Danail and Mateus, Diana and Zuluaga, Maria A. and Zhou, S. Kevin and Racoceanu, Daniel and Joskowicz, Leo",
  title    = "Prediction of Pathological Complete Response to Neoadjuvant Chemotherapy in Breast Cancer Using Deep Learning with Integrative Imaging, Molecular and Demographic Data",
  journal  = "Medical Image Computing and Computer Assisted Intervention – MICCAI 2020",
  booktitle = "Medical Image Computing and Computer Assisted Intervention – MICCAI 2020",
  series    = "MICCAI",
  year      = 2020,
  publisher = "Springer International Publishing",
  address   = "Cham",
  pages = "242--252",
  isbn="978-3-030-59713-9"
}

@article{prostate-cdis,
  author   = "Alexander Wong and Hayden Gunraj and Vignesh Sivan and Masoom A. Haider",
  title    = "Synthetic correlated diffusion imaging hyperintensity delineates clinically significant prostate cancer",
  journal  = "Scientific Reports",
  volume    = {12},
  year      = {2022},
  number    = {3376},
  url       = {https://doi.org/10.1038/s41598-022-06872-7}
}

@misc{public-health-agency,
  title = "Breast Cancer",
  author = "{Public Health Agency of Canada}",
  howpublished = "\url{https://www.canada.ca/en/public-health/services/chronic-diseases/cancer/breast-cancer.html}",
  year = 2019,
  note = "Accessed: 2022-06-02"
}

@article{radiomics,
    title = {Radiomics in breast cancer classification and prediction},
    journal = {Seminars in Cancer Biology},
    volume = {72},
    pages = {238-250},
    year = {2021},
    note = {Precision Medicine in Breast Cancer},
    issn = {1044-579X},
    doi = {https://doi.org/10.1016/j.semcancer.2020.04.002},
    url = {https://www.sciencedirect.com/science/article/pii/S1044579X20300833},
    author = {Allegra Conti and Andrea Duggento and Iole Indovina and Maria Guerrisi and Nicola Toschi},
    keywords = {Radiomics, Breast cancer, Cancer classification, Cancer diagnosis, Cancer prediction.}
}


@misc{sbr-grade-sys,
  title = "Histological Grading of Breast Cancer",
  author = "Robert D. Cardiff and Roy A. Jensen",
  howpublished = "\url{http://tvmouse.ucdavis.edu/bcancercd/311/grading\_diagram.html}",
  note = "Accessed: 2022-12-10"
}

@article{sbr-useful,
  author   = "Sophie Amat  and Frederique Penault-Llorca and Hervew Cure and Guillaume Le Bouedëc and Jean-Louis Achard and Isabelle Van Praagh and Viviane Feillel and Marie-Ange Mouret-Reynier and Jacques Dauplat and Philippe Chollet",
  title    = "Scarff-Bloom-Richardson (SBR) grading: a pleiotropic marker of chemosensitivity in invasive ductal breast carcinomas treated by neoadjuvant chemotherapy",
  journal  = "Int J Oncology",
  volume    = {4},
  year      = {2002},
  pages    = {791-6},
  url       = {https://link.springer.com/article/10.1007/s00428-021-03141-2}
}

@misc{surgery-for-bc,
  title = "Surgery for Breast Cancer",
  author = "{Canadian Cancer Society}",
  howpublished = "\url{https://cancer.ca/en/cancer-information/cancer-types/breast/treatment/surgery}",
  note = "Accessed: 2022-06-02"
}

@article{survival-bc-patients,
  author   = "C. Dimitrakakis and A. Keramopoulos",
  title    = "Survival in primary inoperable breast cancer patients",
  journal  = "European Journal of Gynaecological Oncology",
  year     = 2004,
  volume   = "25",
  number   = "3",
  pages    = "367--372",
}

@article{VM208346402021.72720,
    title = "T1-weighted and T2-weighted MRI image synthesis with convolutional generative adversarial networks",
    journal = "Reports of Practical Oncology and Radiotherapy",
    volume = "26",
    number = "1",
    pages = "35 - 42",
    year = "2021",
    issn = "2083-4640",
    doi = "10.5603/RPOR.a2021.0005",
    url = "https://journals.viamedica.pl/rpor/article/view/RPOR.a2021.0005",
    author = "Daisuke Kawahara and Yasushi Nagata"
}
